Online Test-time Adaptation for 3D Human Pose Estimation: A Practical Perspective with Estimated 2D Poses

Online test-time adaptation for 3D human pose estimation is used for video streams that differ from training data. Ground truth 2D poses are used for adaptation, but only estimated 2D poses are available in practice. This paper addresses adapting models to streaming videos with estimated 2D poses. Comparing adaptations reveals the challenge of limiting estimation errors while preserving accurate pose information. To this end, we propose adaptive aggregation, a two-stage optimization, and local augmentation for handling varying levels of estimated pose error. First, we perform adaptive aggregation across videos to initialize the model state with labeled representative samples. Within each video, we use a two-stage optimization to benefit from 2D fitting while minimizing the impact of erroneous updates. Second, we employ local augmentation, using adjacent confident samples to update the model before adapting to the current non-confident sample. Our method surpasses state-of-the-art by a large margin, advancing adaptation towards more practical settings of using estimated 2D poses.

==> sec/alg.tex <==
\begin{algorithm}[tb]
    \caption{{Overall Adaptation Pipeline}}
    \label{alg:pipeline}
    \begin{algorithmic}[1]
        \REQUIRE Test videos $\mathcal{D}_t = \{V_1, \dots, V_n\}$, pretrained model $\mathcal{M}_{\phi_0}$  
        \STATE $\mathcal{M}_{\phi_1} \leftarrow \mathcal{M}_{\phi_0}$  

        \FOR{$i = 1, \dots, n$}  
            \IF{$\gD_m \neq \emptyset$}  
                \STATE Sample $\{x_1 \dots x_{N_v}\}$ in $\gD_m$ with weights 
                % $\propto 1/\text{selection time}$  
                \STATE 
                $\mathcal{M}_{\phi_i}\leftarrow$
                Update $\mathcal{M}_{\phi_{i-1}}$ via $\gL_{adapt}$ (Eq.~\ref{Eq:adaptive_pl})   
            \ENDIF  
                \STATE  $\mathcal{M}_{\phi_{i1}} \leftarrow \mathcal{M}_{\phi_{i}}$            
            \FOR{$j = 1, \dots, m$}  
            \IF {$j>1$}
                \STATE  $\mathcal{M}_{\phi_{ij}} \leftarrow \mathcal{M}_{\phi_{i(j-1)}}^1$
            \ENDIF
                \IF{$x_{ij}$ is non-conf. \textbf{and} $\exists$ conf. samples in $[j-5,j]$}  
                    \STATE Apply $\ermT_s$ on conf. samples
                    \STATE $\mathcal{M}_{\phi_{ij}}\leftarrow$ Update $\mathcal{M}_{\phi_{ij}}$ via $\gL_{aug}$ (Eq.~\ref{Eq:local_aug})
                \ENDIF  
                \STATE 
                $\{\mathcal{M}_{\phi_{ij}}^1,\mathcal{M}_{\phi_{ij}}^2\}\leftarrow$   Update $\mathcal{M}_{\phi_{ij}}$ via $\gL_{proj}$ (Eq.~\ref{Eq:2d_project}) 
                \STATE $\mathcal{R}\leftarrow$  $\mathcal{M}_{\phi_{ij}}^2(x_{ij})$
                \STATE Pass $\mathcal{M}_{\phi_{ij}}^1$ forward  
            \ENDFOR  

            \STATE Divide $V_i$ into $\mathcal{D}_{\text{conf}}$ and $\mathcal{D}_{\text{non-conf}}$; cluster in each  
            \STATE $\gD_m\leftarrow$  Sample $N_v$ data in $\mathcal{D}_{\text{conf}}$ and $\mathcal{D}_{\text{non-conf}}$ with weights
            % \STATE Store selected samples in 
        \ENDFOR  
        \STATE Calculate MPJPE, PA-MPJPE on $\mathcal{R}$ and GT.
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
% 	\caption{Overall pipeline.}
% 	\label{alg:pipeline}
% 	\begin{algorithmic}[1]
% 	    \REQUIRE Test videos $\mathcal{D}_t = \{V_1, V_2, \ldots, V_n\}$ and pre-trained model $\mathcal{M}_{\phi_0}$ on $\mathcal{D}_s$
%         \STATE{
%             Set $\mathcal{M}_{\phi_{1}} = \mathcal{M}_{\phi_{0}}$ as the initial state for video 1}
%         % \ENSURE Final model
% 		\FOR{$i = 1 ,\dots, n$ videos}
%             \IF{$\gD_m$ is not empty}
%             \STATE{Select $N_v$ samples from $\gD_m$ with weights inversely proportional to their selection time}
%             \STATE{
%             Update initial model from the last video $\mathcal{M}_{\phi_{i-1}}$ with adaptive pseudo-labeling in Eq.~\ref{Eq:adaptive_pl} to obtain $\mathcal{M}_{\phi_{i}}$ 
%             }
%             \STATE{
%             Set $\mathcal{M}_{\phi_{i}}$ as the starting state for the current video
%             }
%             \ENDIF
%                 \FOR{$j = 1 ,\dots, m$ samples}
%                 \IF{$x_{ij}$ is a non-confident sample and is within a 5-interval of confident samples}
%                \STATE{Apply strong augmentation $\ermT_s$ on confident samples within the interval} 
%                \STATE{Update model with local augmentation in Eq.~\ref{Eq:local_aug}}
%                 \ENDIF
%             \STATE{Update model with two-stage optimization in Eq.~\ref{Eq:2d_project} to obtain model states $\mathcal{M}_{\phi_{ij}}^1$ and $\mathcal{M}_{\phi_{ij}}^2$}
%             \STATE{Inference on $x_{ij}$ with $\mathcal{M}_{\phi_{ij}}^2$}
%             \STATE{Pass model state $\mathcal{M}_{\phi_{ij}}^1$ for the next sample}
%                 \ENDFOR
%             \STATE{
%             Split the samples in $V_i$ into confident and non-confident subsets
%             }
%             \STATE{
%             Apply pose clustering in each subset         
%             }
%             \STATE{
%             Select $N_v/2$ in each subset; apply weighted sampling in each cluster
%             }
%             \STATE{
%             Store $N_v$ selected samples in $\gD_m$ 
%             }
% 		\ENDFOR
% 	\end{algorithmic}

% \end{algorithm}
